Testing the Generalization of Neural Language Models for COVID-19 Misinformation Detection

A drastic rise in potentially life-threatening misinformation has been a by-product of the COVID-19 pandemic. Computational support to identify false information within the massive body of data on the topic is crucial to prevent harm. Researchers proposed many methods for flagging online misinformation related to COVID-19. However, these methods predominantly target specific content types (e.g., news) or platforms (e.g., Twitter). The methods' capabilities to generalize were largely unclear so far. We evaluate fifteen Transformer-based models on five COVID-19 misinformation datasets that include social media posts, news articles, and scientific papers to fill this gap. We show tokenizers and models tailored to COVID-19 data do not provide a significant advantage over general-purpose ones. Our study provides a realistic assessment of models for detecting COVID-19 misinformation. We expect that evaluating a broad spectrum of datasets and models will benefit future research in developing misinformation detection systems.

==> tables/finetuned_models_nischals_run.tex <==
\begin{table*}[!htb]
\centering
\caption{F1-Macro scores of neural language models for COVID datasets. The table is divided into three parts: General-Purpose Baselines, Intermediate Pre-Trained, and COVID-19 Intermediate Pre-Trained. \textbf{C}OVID \textbf{A}ware means the model was pre-trained on CORD-19, (\ding{51}) pre-trained on a different dataset (\ding{55}), or the dataset was not reported (\textbf{?}). \textbf{I}ntermediate \textbf{T}raining means the model was pre-trained for a specific domain.
\textbf{Boldface} indicates the highest value for each dataset. $^\dagger$Models already trained on CORD-19. $^*$Large version of the model.} \label{tab:fine_tuned}
\begin{threeparttable}
\resizebox{0.9\textwidth}{!}{
\begin{tabular}{cclcccccr}\toprule
\textbf{IT} & \textbf{CA} & \textbf{Model} & \textbf{CMU-MisCov19} & \textbf{CoAID} & \textbf{ReCOVery} & \textbf{COVID19FN} & \textbf{COVID-CQ} & \textbf{Avg.}      \\
\midrule

%Plain models
- & - & BERT	& 0.35	& 0.94	& 0.75	& 0.66	& 0.75	& 0.69 \\
- & - & RoBERTa & 0.42	& 0.92	& \textbf{ 0.93}	& 0.76	& 0.80	& \textbf{0.77}\\
- & - & BART	& 0.36	&\textbf{ 0.97}	& 0.89	& 0.69	& 0.76	& 0.73\\  
- & - & DeBERTa & 0.47	& 0.93	& 0.84	& 0.67	& 0.78	& 0.74\\ \hdashline\noalign{\vskip 0.5ex}

%specialized models
\ding{51} & - & SciBERT & 0.37	& 0.93	& 0.77	& 0.64	& 0.76	& 0.69\\
\ding{51} & - & BioClinicalBERT	& 0.29	& 0.93	& 0.76	& 0.73	& 0.75	& 0.69\\
\ding{51} & - & BERTweet & 0.03	& 0.67	& 0.40	& 0.66	& 0.71	&0.49\\
\hdashline\noalign{\vskip 0.5ex}

%covid pre-trained models on CORD-19
\ding{51} & \ding{55} & CT-BERT $^*$ & \textbf{0.52}	& 0.94	& 0.82	& 0.66 & \textbf{0.81}	& 0.75 \\
\ding{51} & \textbf{?} & ClinicalCOVID-BERT	& 0.37	& 0.94	& 0.79	& 0.74	& 0.75	& 0.72\\ 
\ding{51} & \textbf{?} & BioCOVID-BERT $^*$	& 0.44	& 0.94	& 0.81	& 0.71	& 0.77	& 0.73\\

\ding{51} & \ding{51} & COVID-BERT $^\dagger$	& 0.36	& 0.93	& 0.78	& 0.74	& 0.76	& 0.71\\
\ding{51} & \ding{51} & COVID-SciBERT $^\dagger$ & 0.34	& 0.94	& 0.78	& 0.67	& 0.76	& 0.70\\
%cord19 by us models in CORD19
\ding{51} & \ding{51} & COVID-RoBERTa	& 0.41	& 0.92	& 0.90	& 0.67	& 0.78	& 0.74\\
\ding{51} & \ding{51} & COVID-BART	& 0.33	& 0.91	& 0.89	& 0.66	& 0.77	& 0.71\\
% \checkmark & - & COVID-Longformer	& 0.00	& 0.48	& 0.40	& 0.36	& 0.00	& 0.25\\
\ding{51} & \ding{51} & COVID-DeBERTa	& 0.33	& 0.93	& 0.89	& \textbf{0.81}	& 0.74	& 0.74\\
% \ding{51} & \ding{51} & CSCT-BERT	& 0.47	& 0.96	& 0.77	& 0.75	& \textbf{0.81}	& 0.75\\ 

\bottomrule
\end{tabular}
}
\end{threeparttable}
\end{table*} 

==> tables/finetuned_weights_covid_cq.tex <==
\begin{table}[!htb]
\centering
\caption{COVID-CQ results of neural language models compared to a baseline. The \textit{static} and \textit{frozen} models use a stacked BiLSTM; \textit{fine-tuned} models were pre-trained on CORD-19 and fine-tuned for the task.}     \label{tab:frozen_weights}
\begin{threeparttable}
\resizebox{0.30\textwidth}{!}{
\begin{tabular}{clr}\toprule
\textbf{Type} &\textbf{Models} & \textbf{F1-Macro}      \\ \midrule
\textit{static} & GloVe    & 0.71   \\ \hdashline\noalign{\vskip 0.5ex}
\textit{frozen} & BERT  & 0.72  \\
\textit{frozen} & RoBERTa & 0.70 \\ 
\textit{frozen} & SciBERT & 0.68 \\\hdashline\noalign{\vskip 0.5ex}
\textit{fine-tuned} & BERT  & \textbf{0.75}  \\
\textit{fine-tuned} & RoBERTa   & \textbf{0.80} \\
\textit{fine-tuned} & SciBERT & \textbf{0.76} \\
\bottomrule
\end{tabular}
}
\end{threeparttable}
\end{table}

==> tables/tokenizer_ablation.tex <==
\begin{table}[!tb]
\centering
\caption{COVID-CQ results of BART and RoBERTa for different \textbf{P}re-\textbf{T}raining and \textbf{F}ine-\textbf{T}uning Tokenizers. All models were pre-trained on the CORD-19 dataset.}\label{tab:tokenizer_inv}
\begin{threeparttable}
\resizebox{0.45\textwidth}{!}{
\begin{tabular}{lllr}\toprule
\textbf{Models} & \textbf{PT Tokenizer} & \textbf{FT Tokenizer}  & \textbf{F1-Macro}     \\ \midrule
RoBERTa	& Standard & Standard	& \textbf{.78}\\
RoBERTa	& COVID & Standard	& .73\\
RoBERTa	& COVID & COVID	& .72\\
BART  & Standard & Standard	& \textbf{.77}\\
BART  & COVID & Standard	& .73\\
BART  & COVID & COVID	& .70\\

\bottomrule
\end{tabular}
}
\end{threeparttable}
\end{table} 
